Interpreting CLIP: Insights on the Robustness to ImageNet Distribution Shifts

What distinguishes robust models from non-robust ones? While for ImageNet distribution shifts it has been shown that such differences in robustness can be traced back predominantly to differences in training data, so far it is not known what that translates to in terms of what the model has learned. In this work, we bridge this gap by probing the representation spaces of 16 robust zero-shot CLIP vision encoders with various backbones (ResNets and ViTs) and pretraining sets (OpenAI, LAION-400M, LAION-2B, YFCC15M, CC12M and {DataComp}), and comparing them to the representation spaces of less robust models with identical backbones, but different (pre)training sets or objectives (CLIP pretraining on ImageNet-Captions, and supervised training or finetuning on ImageNet).Through this analysis, we generate three novel insights. Firstly, we detect the presence of outlier features in robust zero-shot CLIP vision encoders, which to the best of our knowledge is the first time these are observed in non-language and non-transformer models. Secondly, we find the existence of outlier features to be an indication of ImageNet shift robustness in models, since we only find them in robust models in our analysis. Lastly, we also investigate the number of unique encoded concepts in the representation space and find zero-shot CLIP models to encode a higher number of unique concepts in their representation space. However, we do not find this to be an indicator of ImageNet shift robustness and hypothesize that it is rather related to the language supervision. Since the presence of outlier features can be detected without access to any data from shifted datasets, we believe that they could be a useful tool for practitioners to get a feeling for the distribution shift robustness of a pretrained model during deployment.

==> parts/APP_ER.tex <==
\color{blue}
Details on all the models used to calculate slope and intercept of linear model that we use to calculate ER
\color{black}

==> parts/APP_more_layers.tex <==
\subsection{Attention Layers}
\begin{align*}
    W_{OV} = W_O W_V  \hspace{2cm} W_{QK} = W_Q^\intercal W_K
\end{align*}
\begin{align*}
    W_{OV} = \sum_{i=1}^{\rank(W_{OV})}\sigma_i \cdot u_i v_i^{\intercal}
\end{align*}

\begin{align*}
    \importance(i) = \sigma_i \cdot \expect[|\proj{v_i}{H}|] \cdot \expect[|v_i^{\intercal} \ W_{QK} \ H|]
\end{align*}


==> parts/APP_neuron_concepts.tex <==
In our concept analysis in \cref{sec:concept}, we assign concepts to the directions in representation space that are given as the RSVs of the linear head weight matrix $W$. This was motivated by the fact that we discovered that some of those directions are privileged directions emerging from outlier features for robust models, and wanted to understand what information these directions encode. 

However, directions defined by another basis of the representation space can in theory also be used to analyse encoded concepts. In fact, in prior work, individual neurons were used to investigate the concepts encoded by a model \citep{cuadros2022self}, corresponding to the canonical basis of standard unit vectors. We thus replicate the quantitative analysis of \cref{fig:concepts} for the OpenAI zero-shot and finetuned models, but with standard unit vectors $e_i$ replacing $v_i$ in the analysis (for the avoidance of doubt, $e_i$ is defined as a vectors of $0$s, but a $1$ in its $i$-th entry). 

The result is shown in \cref{tab:neuron_uniqueconcepts}.
Again, we see that the more robust zero-shot models encode substantially more unique concepts than the less robust finetuned models. While we did not have enough time to repeat the analysis for all remaining (including superised) models, these intial results make us confident that our concept analysis of \cref{sec:concept} also holds if the basis of directions encoding concepts in representation space were changed to individual neuron directions (or any other basis of $\R^{d_H}$ probably).

%Interestingly, the zero-shot models encode a higher number of concepts though along the RSV directions $v_i$ than the standard unit vector directions $\ve_i$. A deeper analysis of how the changes of basis affects concept encoding would be interesting, but lies beyond the scope of this work.







\begin{table}[t]
\centering
\caption{\emph{Results of the unique concept analysis, showing total $\#$ of unique Broden concepts encoded in last layers along the standard unit vectors $e_i$ of the representation space for models pretrained on OpenAI pretraining data. Zero-shot models encode substantially more concepts.}}
\label{tab:neuron_uniqueconcepts}
\small
\begin{tabular}{lrr}
\toprule
                \multirow{2}*{\textbf{Backbone}}  &  \textbf{Zero-shot CLIP}  &  \textbf{Finetuned CLIP}    \\
         & \emph{Highest ER} & \emph{Medium ER} \\
\midrule
                {ResNet50} &  395 &  331  \\

        {ResNet101}  & 389  &  331   \\

       {ViT-B-16} &     648  &    550  \\

       {ViT-B-32} &   638  &  528   \\


\bottomrule
\end{tabular}
\vspace{-0.4cm}
\end{table}

==> parts/APP_stablerank.tex <==
\color{red}
TO BE UPDATED.
\color{black}

\textbf{Stable rank.} %Just like outliers in the last layer activations alone can not tell the full story of robustness (as there is little difference between finetuned and supervised models, despite their differences in robustness), outliers in the singular values of the classification head matrix $W$ equally do not tell the whole story. This becomes clear in the following 
To detect outliers in the singular values of the classification head matrix $W$, we calculate the stable rank of $W$ defined as 
\begin{equation}
\label{eq:sr}
\text{srank}(W) = \frac{{\sum_{j=1}^{\rank(W)} \sigma_i^2 }}{\sigma_1^2},
\end{equation}
where $\sigma_1$ is the largest singular value of $W$. The results are shown in \cref{tab:sr}.
While we see a clear distinction between the stable rank of the least robust supervised models and the remaining models, there no significant distinction between the most robust zero-shot models and the finetuned models with medium robustness.


\begin{table*}[h]
\centering
\caption{\emph{Results of the stable rank analysis showing outlier singular values of the linear classification head matrix $W$ present in zero-shot models with high robustness and finetuned models with medium robustness, but disappearing for models trained in supervised fashion on ImageNet from scratch. Values calculated according to \cref{eq:sr}. We note that differences between the values for zero-shot and finetuned models do exist, but they only show at the third or fourth digit behind the comma.
%(Shifted ImageNet test sets in brackets).
}}
\label{tab:sr}
\small
\begin{tabular}{llrrr}
\toprule
        \multirow{2}*{\textbf{Backbone}} &  \multirow{2}*{\textbf{Pretraining data}} &  \textbf{Zero-shot CLIP}  &  \textbf{Finetuned CLIP}   & \textbf{ImageNet supervised} \\
        & & \emph{Highest ER} & \emph{Medium ER} & \emph{Lowest ER} \\
\midrule
                \multirow{3}{*}{ResNet50} & OpenAI &  1.30  & 1.30 &  \multirow{3}{*}{8.37} \\
                                  & YFCC-15M &  1.34 & 1.34  &   \\
                                  & CC-12M &  1.40  &  1.40  &  \\ \hline
        \multirow{2}{*}{ResNet101}  & OpenAI & 1.34  &  1.34  &  \multirow{2}{*}{7.57} \\
                                  & YFCC-15M &   1.32  &   1.32 &  \\\hline
       \multirow{4}{*}{ViT-B-16} & OpenAI &     1.27  &    1.27 &  \multirow{4}{*}{ \color{red} tbd  } \\
                                 & LAION-400M & 1.42 &    1.42 &    \\
                                 & LAION-2B &       1.33 &  1.33 &   \\
                                 & DataComp &   1.31   &  1.31  & \\ \hline
        \multirow{4}{*}{ViT-B-32} & OpenAI &   \color{red} tbd   &  \color{red} tbd  & \multirow{3}{*}{ \color{red} tbd } \\
                                  & LAION-400M &  1.29 &  1.29  &  \\
                                  & LAION-2B &   1.34  &   1.34 &   \\ 
                                  \hline
            \multirow{4}{*}{ ViT-L-14} &  OpenAI &   1.39 &  1.39  &   \multirow{4}{*}{ N.A.}   \\
                                     &  LAION-400M &  \color{red} tbd  &  \color{red} tbd    &  \\
                                &  LAION-2B &   1.36  &  1.36  & \\
                                 &  DataComp &     \color{red} tbd &      \color{red} tbd  &  \\ 
                                  %\midrule 
                                  %Average & & \hl{\textbf{XYZ}}  & \hl{\textbf{XYZ}} & \hl{\textbf{XYZ}}  \\
                                  

\bottomrule
\end{tabular}
\vspace{-0.4cm}
\end{table*}

==> parts/impact.tex <==
This paper presents work whose goal is to advance the understanding of robustness in machine learning models. Such an understanding paves the way towards more reliable models, which we believe to have positive societal implications.
